MPC-Pipe: an Efficient Pipeline Scheme for Secure Multi-party Machine Learning Inference

Multi-party computing (MPC) has been gaining popularity as a secure computing model over the past few years. However, prior works have demonstrated that MPC protocols still pay substantial performance penalties compared to plaintext, particularly when applied to ML algorithms. The overhead is due to added computation and communication costs. Prior studies, as well as our own analysis, found that most MPC protocols today sequentially perform communication and computation. The participating parties must compute on their shares first and then perform data communication to allow the distribution of new secret shares before proceeding to the next computation step. In this work, we show that serialization is unnecessary, particularly in the context of ML computations (both in Convolutional neural networks and in Transformer-based models). We demonstrate that it is possible to carefully orchestrate the computation and communication steps to overlap. We propose MPC-Pipe, an efficient MPC system for both training and inference of ML workloads, which pipelines computations and communications in an MPC protocol during the online phase. MPC-Pipe proposes three pipeline schemes to optimize the online phase of ML in the semi-honest majority adversary setting. We implement MPC-Pipe by augmenting a modified version of CrypTen, which separates online and offline phases. We evaluate the end-to-end system performance benefits of the online phase of MPC using deep neural networks (VGG16, ResNet50) and Transformers using different network settings. We show that MPC-Pipe can improve the throughput and latency of ML workloads.

==> archive/evaluation_old.tex <==
\subsection{Experimental Setups}
We have evaluated our design on servers with an Intel Xeon Gold 5220R CPU and an Nvidia Quadro RTX 5000. Implementation of MPC-Pipe is based on CrypTen~\cite{crypten2020}, an MPC framework based on PyTorch from Meta AI. We gather inference runtime from the average of \textbf{50} iterations of inferences so as to remove the influence of random network fluctuations.

\subsection{Enhanced CrypTen Baseline}
We choose a modified CrypTen~\cite{crypten2020} as our baseline.  CrypTen is based on PyTorch, and it supports efficient large-scale operations on GPUs. From our preliminary studies, the usage of GPUs can speed up local operations 5-7 times. Evaluating MPC-Pipe on frameworks with GPU support can give us more realistic performance benefits of MPC-Pipe since ML models are more likely to run on GPUs. Other frameworks like~\cite{kumar2020cryptflow, delphi, mp-spdz, gazzele, chameleon, secureml, fis} neither use semi-honest security nor fully support GPUs. Thus, we choose CrypTen for its full support on GPUs and its support of the semi-honest threat model.

\textbf{Separation of Beaver Triple Generation from the online phase:} The original CrypTen does not separate the offline (Beaver Triple generation) and the online phase. Operators in CrypTen will first request Beaver Triple before running online operations.  We modified CrypTen to separate the offline phases from the online phases. This modified CrypTen that decoupled the offline and online phases is used as the baseline in our experiments. We then implemented all the pipeline schemes on top of the modified Crypten framework to measure the performance of the MPC-Pipe. 

\begin{figure*}[htbp]
  \centering
  \begin{subfigure}[tb]{0.3\linewidth}
    \includegraphics[width=\linewidth]{figures/Vgg16-throughput-10Gbps-Inference.pdf}
    \caption{VGG16 Inference}
    \label{fig:vgg16-throu-lan}
  \end{subfigure}
  \begin{subfigure}[tb]{0.3\linewidth}
    \includegraphics[width=\linewidth]{figures/resnet-throughput-10Gbps-Inference.pdf}
    \caption{ResNet Inference}
    \label{fig:resnet-throu-lan}
  \end{subfigure}
    \begin{subfigure}[tb]{0.3\linewidth}
    \includegraphics[width=\linewidth]{figures/xformer-throughput-10Gbps-Inference.pdf}
    \caption{Transformer Inference}
    \label{fig:xformer-throu-lan}
  \end{subfigure}
  \label{fig:worst-speedups}
  \begin{subfigure}[tb]{0.30\linewidth}
    \includegraphics[width=\linewidth]{figures/Vgg16-throughput-10Gbps-Train.pdf}
    \caption{VGG16 Training}
    \label{fig:vgg16-throu-wan}
  \end{subfigure}
  \begin{subfigure}[tb]{0.30\linewidth}
    \includegraphics[width=\linewidth]{figures/resnet-throughput-10Gbps-Train.pdf}
    \caption{ResNet Training}
    \label{fig:resnet-throu-wan}
  \end{subfigure}
  \begin{subfigure}[tb]{0.30\linewidth}
    \includegraphics[width=\linewidth]{figures/xformer-throughput-10Gbps-Train.pdf}
    \caption{Transformer Training}
    \label{fig:xformer-throu-wan}
  \end{subfigure}
  \caption{MPC-Pipe Throughput Performance Benefits.}
  \label{fig:throuputs}
\end{figure*}

\subsection{Methodology}
We conducted tests to evaluate the impact of MPC-Pipe on inference throughput and latency in two settings: 2PC (with two MPC servers) and 3PC (with three MPC servers). We consider 2PC and 3PC to be robust security models that can tolerate one or two compromised MPC servers while keeping hardware costs and performance overheads low. While we did not evaluate MPC-Pipe in the 3+PC setting, we provide a quantitative analysis of its scaling capabilities in section~\ref{sec:more-parties}. We also tested MPC-Pipe on six different network configurations, including LAN and WAN connections at three different speeds (10Gbps, 20Gbps, and 40Gbps). In the LAN setting, communication cost mainly consists of data transmission time (file size $/$ bandwidth) while in the WAN setting, communication cost consists of both data transmission time and data propagation delay (time taken for a bit to travel from the source server to the destination server). In the WAN setting, the network propagation time was approximately 70ms.

\subsubsection{Models evaluated}
We evaluated MPC-Pipe on two major Machine Learning workloads: 1) a Transformer-based model and 2) Convolution Neural Networks. The Transformer architecture we selected is the one used in popular Natural Language Processing models \cite{bert, roberta, xlm, xlmr}, and the CNN models we selected are VGG16\cite{vgg} and ResNet50\cite{resnet}.

\subsection{Throughput}
In this section, we will demonstrate how MPC-Pipe can enhance the throughput performance of Machine Learning inference. Throughput refers to the number of inputs that can undergo model inference within a unit of time. Figure~\ref{fig:throuputs} illustrates the throughput enhancements achieved by MPC-Pipe, with a connection bandwidth of 10Gbps, over the enhanced Crypten baseline that decouples online and offline phases. The data in the first row of the figures were collected in the LAN setting, while the data in the second row were collected in the WAN setting. Each figure shows the 2PC and the 3PC setting results. 
The first and fourth bar (label "$+$Pipe") in each subfigure displays the throughput improvement achieved by applying only inter-linear and inner-layer pipeline. The second and fifth bar (labeled "$+$Para") shows the throughput improvement achieved by applying only the inter-batch pipeline (3rd scheme) during inference, which overlaps linear and nonlinear layers for different mini-batches.  The third and sixth bars (labeled "$+$MPC-Pipe") represent the throughput enhancement achieved by applying all pipeline schemes during inference. 

\subsubsection{CNN Models}
Figures~\ref{fig:vgg16-throu-lan},~\ref{fig:vgg16-throu-wan},~\ref{fig:resnet-throu-lan}, and~\ref{fig:resnet-throu-wan} demonstrate the improvement in throughput achieved by MPC-Pipe for VGG16 and ResNet50, respectively. When using only the inter-linear and inner-layer pipelines, which shorten the inference runtime of individual layers, MPC-Pipe provides a throughput improvement of approximately $10\%$ (further details on latency can be found in Section \ref{sec:exp-latency}). By applying solely the inter-batch pipeline  to CNN models, MPC-Pipe increases the throughput by up to $22\%$. 
The inter-batch pipeline technique is designed to increase the throughput of ML models by overlapping the runtime of linear and non-linear layers. However, the improvement in throughput is limited by the percentage of total inference time taken up by the linear layers. This is because linear layers tend to execute faster than the non-linear layers with which they are pipelined. 
Table~\ref{tab:linear-percent} shows the detailed percentage of runtime that is taken up by the linear layers in the $2$PC setting. When using a LAN, both VGG16 and ResNet's linear layer runtime is about $33\%$ of total runtime. Due to GPU resource contention, a perfect $33\%$ throughput cannot be achieved. When using a WAN, VGG16's linear runtime percent decreases more than that of ResNet because there are more non-linear operations per convolutions in VGG16 (ReLU and MaxPool) than in ResNet (only ReLU). Thus, when using the WAN, VGG16 sees lesser speedups than ResNet. When MPC-Pipe applies all the pipeline schemes to CNN models, their runtime is reduced by around $33\%$ because the inner-layer pipeline or the inter-linear pipeline will further reduce the layer runtime that bottlenecks the pipeline. For both CNN models, when moving from the 2PC to the 3PC setting, the throughput improvement is roughly the same. In the 3PC setting, the linear layer's percentage of the runtime is reduced to around $25\%$ in the LAN setting. However, due to the longer data transmission time of non-linear layers, there is less contention over GPU usage. Thus, in the 3PC setting, the throughput improvement solely using the inter-batch pipeline is closer to the ideal throughput reduction.


\begin{table}[h]
\centering
\caption{Linear Runtime \% of 2PC Inference Runtime w/ 10Gbps.}
\label{tab:linear-percent}
\begin{tabular}{|c|c|rr|}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{Components} & \multicolumn{2}{c|}{\% of Runtime} \\ \cline{3-4} 
                  &                             & \multicolumn{1}{r|}{LAN}   & WAN   \\ \hline
VGG16             & Conv2D                      & \multicolumn{1}{r|}{33\%}  & 26\%  \\ \hline
ResNet50          & Conv2D, BatchNorm           & \multicolumn{1}{r|}{33\%}  & 30\%  \\ \hline
Xformer           & Dense, Matmul               & \multicolumn{1}{r|}{42\%}  & 32\%  \\ \hline
\end{tabular}
\end{table}


\subsubsection{Transformers}
\label{sec:eval-through-xformer}
Figures~\ref{fig:xformer-throu-lan} and~\ref{fig:xformer-throu-wan} show the throughput improvement of MPC-Pipe for the Transformer model. The naming convention is the same as other subfigures in Figure~\ref{fig:throuputs}. When using only the inter-linear and inner-layer pipelines, which shorten the inference runtime of individual layers, MPC-Pipe provides a throughput improvement of approximately $12\%$ (further details on latency can be found in Section \ref{sec:exp-latency}). As for the inter-batch pipeline, MPC-Pipe also needs to overlap the linear and non-linear operations of Transformers. Unlike CNNs, Transformers' inter-batch pipeline is relatively unbalanced. Although data in Table~\ref{tab:linear-percent} shows that the percentage of linear runtime of Transformer is closer to 50$\%$, Transformer's specific architecture makes inter-batch pipeline less efficient. Unlike CNNs' architecture, each linear layer is followed by a non-linear layer, in each Transformer layer, there are $5$ Dense layers, one Softmax, and 1 ReLU. Due to the positioning of non-linear layers, the ratio of linear and non-linear layers pipelined together is about $\frac{1}{3}$ (the ratio for CNN is about $\frac{1}{2}$). Thus,  the inter-batch pipeline's efficiency is relatively low compared with CNN models. When moving from the LAN setting to the WAN setting, the Transformer sees fewer benefits from MPC-Pipe because Softmax requires more rounds of communications than ReLU and MaxPool.

When moving from the 2PC setting to the 3PC setting, MPC-Pipe gives Transformers more improvements. This is because, in the Softmax function, there are nine iterations of comparisons to find a maximum along one dimension. There are some iterations of comparisons whose communication overhead is smaller than the computation overhead, although the total communication cost of Softmax is higher than the total computation cost. Thus, for those iterations with smaller communication overhead, in the 3PC setting, the pipeline can be better balanced, resulting in better latency improvement.
% \begin{figure}[h]
%   \centering
%     \includegraphics[width=6cm]{figures/ThroughputVSpeed.pdf}
%   \caption{MPC-Pipe's Throughput Improvements with Faster Connections.}
%   \label{fig:throuVspeed}
% \end{figure}

% \subsubsection{Throughput Improvement with Faster Connections}
% Figure~\ref{fig:throuVspeed} shows the MPC-Pipe's throughput improvement using 3 interconnection bandwidths (10Gbps, 20Gbps, 40Gbps). In the LAN setting, with faster connections, MPC-Pipe's performance benefit decreases while in the WAN setting, the performance benefit roughly stays the same. Note that in the WAN setting the propagation delay is about 70 ms.  Recall from the previous discussion, throughput improvements are bounded by the percentage of the layer in the pipeline that has shorter runtime. With faster connections, the non-linear layer's runtime in the LAN setting becomes shorter than that of the linear layers such that there are fewer communications  to be hidden resulting in fewer speedups. In the WAN setting, there are still enough communications for linear operations to hide resulting in roughly the same performance benefit.




% Since MPC-Pipe targets overlapping communication with computations, it is naturally more beneficial in network conditions where bandwidth is a constraint. In our LAN setting the MPC servers were all hosted in a single rack and were able to communicate over a rack switch. Hence in such conditions network contention was limited, which limited MPC-Pipe to 20\% throughput improvements, which is still substantial.  


\begin{figure*}[htbp]
  \centering
  \begin{subfigure}[tb]{0.3\linewidth}
    \includegraphics[width=\linewidth, height=3.5cm]{figures/Vgg-latency-10Gbps-Inference.pdf}
    \caption{VGG16 Inference}
    \label{fig:vgg16-lat-infer}
  \end{subfigure}
  \begin{subfigure}[tb]{0.3\linewidth}
    \includegraphics[width=\linewidth, height=3.5cm]{figures/ResNet-latency-10Gbps-Inference.pdf}
    \caption{ResNet Inference}
    \label{fig:resnet-lat-infer}
  \end{subfigure}
    \begin{subfigure}[tb]{0.3\linewidth}
    \includegraphics[width=\linewidth, height=3.5cm]{figures/xformer-latency-10Gbps-Inference.pdf}
    \caption{Transformer Inference}
    \label{fig:xformer-lat-infer}
  \end{subfigure}
  \label{fig:worst-speedups}
  \begin{subfigure}[tb]{0.30\linewidth}
    \includegraphics[width=\linewidth, height=3.5cm]{figures/Vgg-latency-10Gbps-Train.pdf}
    \caption{VGG16 Training}
    \label{fig:vgg16-lat-train}
  \end{subfigure}
  \begin{subfigure}[tb]{0.30\linewidth}
    \includegraphics[width=\linewidth, height=3.5cm]{figures/ResNet-latency-10Gbps-Train.pdf}
    \caption{ResNet Training}
    \label{fig:resnet-lat-train}
  \end{subfigure}
  \begin{subfigure}[tb]{0.30\linewidth}
    \includegraphics[width=\linewidth, height=3.5cm]{figures/xformer-latency-10Gbps-Train.pdf}
    \caption{Transformer Training}
    \label{fig:xformer-lat-train}
  \end{subfigure}
  \caption{MPC-Pipe Latency Performance Benefits.}
  \label{fig:latency}
\end{figure*}


\subsection{Latency}
\label{sec:exp-latency}
In this section, we will showcase MPC-Pipe's latency performance benefits for Machine Learning inference. Latency is defined as the time taken from a model receiving an input to the model producing the final result for that input. The inter-linear pipeline and the inner-layer pipeline techniques are targeted to  shorten the latency of individual layers while the inter-batch pipeline focused on improving the throughput.

\subsubsection{CNN Models}
\label{sec:cnn-lat}
In this section, we present MPC-Pipe's performance benefits for CNN model inference by breaking down the computation of CNN models into three main categories: 1) Linear, 2) ReLU, and 3) MaxPool. The Linear category includes Convolution layers in feature abstraction layers and Dense layers in classifiers, with most of the Linear layers being Convolutions.  VGG16 has 5 Maxpooling layers and ResNet50 has none.

Figures~\ref{fig:vgg16-lat-lan},~\ref{fig:vgg16-lat-wan},~\ref{fig:resnet-lat-lan}, and ~\ref{fig:resnet-lat-wan} demonstrate the latency improvement of MPC-Pipe for VGG16 and ResNet50. The left part of each figure shows the latency improvement in the 2PC settings, while the right part shows the latency improvement in the 3PC setting. 

In the 2PC LAN setting, MPC-Pipe provides $10.9\%$ latency improvement for VGG16 and $10.6\%$ for ResNet50. In the 3PC LAN setting, MPC-Pipe provides $13.3\%$ and $10.4\%$ latency improvements for VGG16 and ResNet50, respectively. Linear operations' latency mainly benefits from the inter-layer pipeline to hide communication of weight metadata, whereas Maxpooling and ReLU's latency benefits mainly from the inner-layer pipeline. When transitioning from the 2PC setting to the 3PC setting, MPC-Pipe's performance benefit to VGG16 increases, while the benefit to ResNet50 remains roughly the same. The main reason for the increase in benefit to VGG16 is due to the MaxPool operations. For MaxPool, when moving from the 2PC to the 3PC setting, the increase in computation workload outweighs the increase in communication, allowing more computation to be hidden and resulting in better performance benefits. Better performance benefits for the MaxPool gives VGG16 better latency improvements in 3PC.

When moving from the LAN setting to the WAN setting, non-linear layers see fewer performance benefits, while linear layers continue to see significant gains. This is because all the linear layers are computation-dominant, and the increased communication costs from network latency result in more performance improvements.


\subsubsection{Transformers}
In this section, we will demonstrate MPC-Pipe's impact on Transformer inference latency. We break Transformer computations into four main categories: 1) Linear, 2) Softmax, 3) ReLU, and 4) Attention.  The Attention layer includes the two matrix multiplications in Multi-headed Attention computation. The linear category includes all other matrix multiplications in the Transformers. The linear operations in the Transformers mainly benefit from the inter-linear pipeline. Other operations mainly benefit from the inner-layer pipeline. Both Softmax and ReLU operations benefit from load balancing due to their use of the SPK circuit.

Figures~\ref{fig:xformer-lat-lan} and~\ref{fig:xformer-lat-wan} show latency improvement for each component of Transformers. The left part shows the latency improvement in the $2$PC setting, and the right part shows the latency improvement in the $3$PC setting. In the LAN setting, MPC-Pipe brings $10.6\%$ and $13.5\%$ latency improvement in the 2PC and the 3PC setting, respectively. In the WAN setting, the latency improvements are $7.4\%$ and $11.9\%$, respectively, in the 2PC and the 3PC setting. Latency improvement grows with the number of parties -- $3$PC setting has better latency improvement than $2$PC.  The reasoning is the same as that in Section~\ref{sec:eval-through-xformer}. When moving from the LAN setting to the WAN setting, every component shows a similar trend as we observed in Section~\ref{sec:cnn-lat}.

\subsection{MPC-Pipe with Nvidia H100}
% We also collect the performance improvement of MPC-Pipe with the most powerful GPU ever: Nvidia H100. Table~\ref{tab:h100res} shows the throughput and latency improvements of MPC-Pipe with Nvidia H100. MPC-Pipe continues to demonstrate great performance despite the usage of a much more powerful GPU. MPC-Pipe will hide the runtime for communication for linear layers, and hide the runtime for computations for non-linear layers. With a faster GPU, MPC-Pipe's runtime reduction for linear layers stays the same, and that of non-linear layers decreases. Furthermore, due to the usage of a faster GPU, the runtime of our baseline also reduces. Because of this, although the total runtime reduction for MPC-Pipe is reduced due to Nvidia H100, MPC-Pipe can still demonstrate significant performance improvements over the baseline.
\textcolor{blue}{We have also evaluated the performance improvement of MPC-Pipe using the most advanced GPU available, the Nvidia H100. As depicted in Table~\ref{tab:h100res}, there are clear throughput and latency benefits when utilizing MPC-Pipe with the Nvidia H100. MPC-Pipe maintains its performance even when paired with this significantly more powerful GPU. MPC-Pipe effectively masks the runtime of communication for linear layers and the computational runtime for non-linear layers. When equipped with a faster GPU like the Nvidia H100, the runtime reduction attributed to linear layers remains consistent, while that for non-linear layers diminishes slightly. Moreover, the runtime for our baseline model also sees a reduction due to the enhanced processing power of the GPU. Therefore, even though the total runtime reduction for MPC-Pipe is somewhat lessened with the Nvidia H100, it still manages to achieve notable performance gains over the baseline.}

\begin{table}[h]
    \centering
    \caption{MPC-Pipe's Performance Improvement with Nvida-H100.}
    \begin{tabular}{|ll|r|r|r|}
        \hline
        \multicolumn{2}{|l|}{}                                        & \multicolumn{1}{c|}{Xformer} & \multicolumn{1}{c|}{VGG16} & \multicolumn{1}{c|}{ResNet} \\ \hline \hline
        \multicolumn{1}{|l|}{\multirow{2}{*}{Inference}} & Throughput & $26\%$                       & $17\%$                     & $16\%$                      \\ \cline{2-5} 
        \multicolumn{1}{|l|}{}                           & Latency    & $11\%$                       & $9.7\%$                    & $4.5\%$                     \\ \hline \hline
        \multicolumn{1}{|l|}{\multirow{2}{*}{Training}}  & Throughput & $25\%$                    & $23\%$                  & $14\%$                   \\ \cline{2-5} 
        \multicolumn{1}{|l|}{}                           & Latency    & $9.8\%$                     & $16\%$                  & $9.7\%$                     \\ \hline
    \end{tabular}
    \label{tab:h100res}
\end{table}

% In the Softmax function, there are $9$ iterations of comparisons to find a maximum along one dimension. There are some iterations of comparisons whose communication overhead is smaller than the computation overhead, although the total communication cost of Softmax is higher than the total computation cost. Thus, for those iterations with smaller communication overhead, in the $3$PC setting, the inner-layer pipeline can be better balanced, resulting in better latency improvement.

% \subsubsection{Latency Improvement with Faster Connections}
% Figure~\ref{fig:latVspeed} shows the MPC-Pipe's latency improvement using 3 interconnection bandwidths (10Gbps, 20Gbps, 40Gbps). In contrast to what we have seen in Figure~\ref{fig:throuVspeed}, MPC-Pipe's latency improvements decrease in the WAN setting with faster connections while that of the LAN setting roughly stays the same. Latency improvements are mainly derived from hiding communications and computations within individual Machine Learning layers. In the LAN setting with faster communications, communications in both linear and nonlinear layers are becoming faster. For linear layers, the decrease in communication will result in fewer improvements because linear layers are computationally dominant. For non-linear layers, faster communication will result in better improvements. The treads in linear and nonlinear layers roughly cancel each other out resulting in similar improvements when using faster interconnections.


% \begin{figure}[h]
%   \centering
%     \includegraphics[width=6cm]{figures/LatencyVSpeed.pdf}
%   \caption{MPC-Pipe's Latency Improvements with Faster Connections.}
%   \label{fig:latVspeed}
% \end{figure}

\subsection{MPC-Pipe with Different Connection Speed}

\begin{table}[h]
\centering
\caption{Throughput of MPC \& MPC-Pipe w/ different LAN speed in input/minute; ``Pipe'' column denotes throughput of MPC-Pipe}
\begin{tabular}{|l|rr|rr|rr|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Inference}} & \multicolumn{2}{c|}{VGG16}                            & \multicolumn{2}{c|}{ResNet}                            & \multicolumn{2}{c|}{Xformer}                           \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                           & \multicolumn{1}{c|}{MPC}  & \multicolumn{1}{c|}{Pipe} & \multicolumn{1}{c|}{MPC}   & \multicolumn{1}{c|}{Pipe} & \multicolumn{1}{c|}{MPC}   & \multicolumn{1}{c|}{Pipe} \\ \hline
10Gbps                                           & \multicolumn{1}{r|}{4.21} & 6.31                      & \multicolumn{1}{r|}{9.00}  & 13.55                     & \multicolumn{1}{r|}{10.52} & 13.93                     \\ \hline
20Gbps                                           & \multicolumn{1}{r|}{6.42} & 8.84                      & \multicolumn{1}{r|}{13.77} & 19.93                     & \multicolumn{1}{r|}{14.86} & 18.94                     \\ \hline
40Gbps                                           & \multicolumn{1}{r|}{8.14} & 10.13                     & \multicolumn{1}{r|}{18.70} & 24.43                     & \multicolumn{1}{r|}{18.07} & 22.30                     \\ \hline
\end{tabular}
\label{tab:throuVspeed}
\end{table}
Table~\ref{tab:throuVspeed} shows the throughput of MPC and MPC-Pipe for different models using different interconnection speeds in the LAN setting. Most noticeably, the throughput of MPC-Pipe using 10Gbps is similar to baseline MPC using 20Gbps. For instance, the throughput of VGG16 using 20Gbps is 6.31 inputs/minute, and the throughput of VGG16 on MPC-Pipe using 10Gbps is 6.42 inputs/minute. A similar observation is true for baseline MPC using 40Gbps LAN and MPC-Pipe using 20Gbps LAN. Thus,  MPC-Pipe becomes even more advantageous in congested network settings. We observed similar trends for MPC-Pipe with WAN interconnection. 


\begin{table}[h]
\centering
\caption{Latency of MPC \& MPC-Pipe w/ different LAN speed in second; ``Pipe'' column denotes latency of MPC-Pipe}
\begin{tabular}{|c|cc|cc|cc|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{VGG16} & \multicolumn{2}{c|}{ResNet} & \multicolumn{2}{c|}{Xformer}          \\ \cline{2-7} 
                  & \multicolumn{1}{c|}{MPC}  & Pipe & \multicolumn{1}{c|}{MPC}   & Pipe & \multicolumn{1}{c|}{MPC}   & Pipe \\ \hline
10Gbps            & \multicolumn{1}{c|}{14.25} & 12.7 & \multicolumn{1}{c|}{6.66} & 5.96 & \multicolumn{1}{c|}{5.78} & 5.17 \\ \hline
20Gbps            & \multicolumn{1}{c|}{9.6}   & 8.59 & \multicolumn{1}{c|}{4.36} & 3.92 & \multicolumn{1}{c|}{4.03} & 3.67 \\ \hline
40Gbps            & \multicolumn{1}{c|}{7.36}  & 6.71 & \multicolumn{1}{c|}{3.21} & 2.86 & \multicolumn{1}{c|}{3.32} & 3.02 \\ \hline
\end{tabular}
\label{tab:latVspeed}
\end{table}

Table~\ref{tab:latVspeed} shows the latency of MPC and MPC-Pipe for different models using different interconnection speeds in the LAN setting. MPC with 20Gbps is about 30\% faster than MPC-Pipe with 10Gbps. But when the bandwidth increases to 40 Gbps for the baseline MPC, MPC-Pipe with half the bandwidth of 20Gbps is only 10\% slower than the baseline with 40Gbps. Hence, at a higher bandwidth regime, MPC-Pipe is going to be nearly as quick as baseline MPC with 2X the bandwidth. Based on the data from the above two tables, we conclude that when bandwidth is constrained, MPC-Pipe provides good throughput benefits, and when bandwidth is more, MPC-Pipe will provide similar latency as the baseline with just half the bandwidth needed.

\subsection{Support for Training}
\textcolor{blue}{Our proposed approach will also work for training operations. Backward operations for non-linear layers like ReLU and MaxPooling are element-wise multiplication. For example, the ReLU backward function will be element-wise multiplication between a secret shared input mask and output gradients. The input mask indicates which elements in the original inputs are non-zero. In such a case, the inner-layer pipeline will be applicable.}

\textcolor{blue}{For linear layers, backward operations involve matrix multiplication, such as in fully connected layers, where the backward function requires multiplying output gradients with both the input and weight matrices ($x^T \cdot grad_{out}$ and $grad_{out} \cdot w^T$). After the forward pass, both matrices ($x$ and $w$) are available. During the backward pass, MPC parties utilize the inter-linear pipeline to obscure communication concerning these matrices. Our experiments show that using both inter-linear and inner-layer pipelines can reduce latency by 10\%-14\% for these operations}

\subsection{Scaling beyond 3 parties}
\label{sec:more-parties}


MPC-Pipe is built on generalized MPC protocols that are not limited to a specific number of parties. Hence, they can functionally scale to multiple MPC servers. In the previous sections, we quantified MPC-Pipe's advantages in both 2PC and 3PC settings. Due to infrastructure limitations, we limited our detailed quantitative analysis to the 3PC setting. This section provides a qualitative analysis with some analytical model data for explaining the scalability of MPC-Pipe with the 3$+$PC setting. 
To understand the scalability, Figure~\ref{fig:bytes} plots the total bytes sent and received by an MPC server as we scale to the 3$+$PC settings for both VGG and ResNet. The number of total bytes increases linearly as we scale to the 3$+$PC settings. In the 3PC setting for VGG16, roughly 17GB of data is sent and received by a single party, while in the 4PC setting, it is about 25GB. In a distributed computing setting, such as MPC, as the total bytes of communication increases it is expected that the underlying interconnection fabric also scales.  For instance, 2PC VGG with 10Gbps link takes about 17 seconds per inference. If one uses the same 10Gbps link with a 4PC setting then the transmission of 25GB of data takes nearly 20 seconds just to communicate the data (assuming no network contention). Thus, if one does not scale interconnection bandwidth with the number of MPC servers, the system will be bounded by the communication bottleneck. Thus, increasing the MPC servers without increasing the interconnection bandwidth makes MPC less performant. Consequently, in our scaling analysis, we make the assumption that as we scale to more parties, we will also linearly scale the bandwidth of the interconnections between MPC servers. For instance, for the 3PC setting, we assume the interconnection bandwidth is 20Gbps, and 4PC has 30 Gbps bandwidth. Under this scenario, MPC-Pipe can overlap the computation and communication phases effectively, as we have demonstrated. In fact, the results in Table~\ref{tab:past} demonstrate this fact. We show the performance improvement of MPC-Pipe in the 2PC (with a 10Gbps interconnection) and 3PC (with a 20Gbps interconnection) settings in Table~\ref{tab:past}. MPC-Pipe's latency and throughput benefits remain roughly the same, scaling from 2PC to 3PC with scaled-up interconnection bandwidth. Based on these assumptions, we believe the MPC-Pipe's performance benefits with more MPC servers will remain stable.
\begin{figure}[h]
  \centering
    \includegraphics[width=8cm]{figures/bytes.pdf}
  \caption{Total Bytes Sent and Received by an MPC Server.}
  \label{fig:bytes}
\end{figure}

\begin{table}[h]
\caption{MPC-Pipe Performance Benefits for 2PC and 3PC w/ scaled up bandwidth.}
\label{tab:past}
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{VGG16} & \multicolumn{2}{c|}{ResNet} \\ \cline{2-5} 
                  & \multicolumn{1}{c|}{Throughput} & Latency & \multicolumn{1}{c|}{Throughput}     & Latency      \\ \hline
2PC 10Gbps LAN & \multicolumn{1}{c|}{33.2$\%$}       & 10.9$\%$    & \multicolumn{1}{c|}{33.5$\%$}       & 10.6$\%$     \\ \hline
3PC 20Gbps LAN & \multicolumn{1}{c|}{28.7$\%$}       & 11.2$\%$    & \multicolumn{1}{c|}{29.2$\%$}       & 10.7$\%$     \\ \hline
2PC 10Gbps WAN & \multicolumn{1}{c|}{30.0$\%$}       & 9.7$\%$    & \multicolumn{1}{c|}{30.9$\%$}       & 10.6$\%$     \\ \hline
3PC 20Gbps WAN & \multicolumn{1}{c|}{27.5$\%$}       & 9.4$\%$    & \multicolumn{1}{c|}{29.1$\%$}       & 11.8$\%$     \\ \hline
\end{tabular}
\end{table}
